F-FADE: Frequency Factorization for Anomaly Detection in Edge Streams

Edge streams are commonly used to capture interactions in dynamic networks, such as email, social, or computer networks. The problem of detecting anomalies or rare events in edge streams has a wide range of applications. However, it presents many challenges due to lack of labels, a highly dynamic nature of interactions, and the entanglement of temporal and structural changes in the network. Current methods are limited in their ability to address the above challenges and to efficiently process a large number of interactions. Here, we propose F-FADE, a new approach for detection of anomalies in edge streams, which uses a novel frequency-factorization technique to efficiently model the time-evolving distributions of frequencies of interactions between node-pairs. The anomalies are then determined based on the likelihood of the observed frequency of each incoming interaction. F-FADE is able to handle in an online streaming setting a broad variety of anomalies with temporal and structural changes, while requiring only constant memory. Our experiments on one synthetic and six real-world dynamic networks show that F-FADE achieves state of the art performance and may detect anomalies that previous methods are unable to find.

==> 050discussion.tex <==
\section{Discussion (Benefit)}
\begin{itemize}
\item embedding-based methods -> community, generalization, more robust 
\item local update -> efficient
\item Aggregate a set of events 
\end{itemize}

\begin{itemize}
\item Either communicating more or less frequently than usual (frequency), or communicating with different individuals than usual (community).~\cite{heard2010bayesian}. Compare to \cite{heard2010bayesian}, counting process + markov, discrete time, no embedding
\item Compare to PageRank~\cite{yoon2019fast}, continuous time, theoretical description
\item Compare to MIDAS~\cite{bhatia2020midas}, community level
\item Compare to local~\cite{liu2019real}, more fit for anomaly detection, 
\item Compare to Spotlight~\cite{eswaran2018spotlight}: Lemma 5.1 (Star vs. matching); Theorem 5.2 (Focus-Awareness) can be proved; no community
\item Compare to Sedanspot\cite{eswaran2018sedanspot}: consider topology via PageRank; no statistical 

\end{itemize}


==> 060related.tex <==
\section{Related works: Different types of anomalies in edge streams}
Sedanspot~\cite{eswaran2018sedanspot}: burst behavior + connect a sparse graph (PageRank)
MIDAS~\cite{bhatia2020midas}: burst behavior + Microcluster 
local-detection + local-update, in a more real-time detection (less delay and more accurate), not good to detect deletion 

edge level+ decomposition + local update + statistical control

Graph level:
Spotlight~\cite{eswaran2018spotlight}: connect/delete a dense graph
PageRank~\cite{yoon2019fast}:  burst behavior + connect/delete a dense graph 

preNetwalk~\cite{yu2017temporally}: decomposition + auto regression
NetWalk~\cite{yu2018netwalk}: like decomposition based (more community related)
hypersphere~\cite{teng2017anomaly}: like decomposition
hotspot discovery~\cite{yu2013anomalous}: local decomposition (one related baseline)
dense region~\cite{mongiovi2013netspot}: only based on counting, no comparison 

\cite{hu2016embedding,aggarwal2012event}: community + embedding/clustering

survey~\cite{ranshous2015anomaly,cadena2018graph}


Scan statistics~\cite{chen2014non}: record the full record, global behavior, with feature
partition + edge likelihood~\cite{aggarwal2011outlier}


(static) Changepoint: Scan statistics~\cite{sharpnack2013changepoint,sharpnack2013near}: densely connected graph (too specific model assumption)
(static) less-is-more~\cite{sun2007less}: efficient decomposition 




\cite{peel2015detecting}: full model, global behavoir 







% Our  goal  is  to  detect  anomalous  edges  by  leveraging  theirtemporal  and  spatial  signals,  i.e.,  they  tend  to  (i)  occur  asbursts of activity and (ii) connect sparsely-connected parts ofthe graph. To do this quickly using bounded memory, we main-tain a fixed-size sample of the edges seen thus far and use itto score the anomalousness of any new edge. Thus, Problem 1can  be  subdivided  into  two  subproblems,  each  incorporatingone of the above signals of anomalousness, as follows:Informal Problem 2 (Edge sampling).Given an edge streamEandS∈N, maintain an online sampleSofSedges whiledownsampling bursts of activity.Informal Problem 3 (Anomaly scoring).Given a sample ofedgesSand a new edgeei, design an anomaly scoring func-tionyi=f(ei;S)to give a higher score to edges connectingparts of the graph which are sparsely connected.



% %= \{(v_i, u_i, t_i)\in \mathcal{E}| t_i\leq t \}$
% %. Therefore, $V_t$ and $\mathcal{E}_t$ increase with respect to the time $t$.



% $V_t$ contains all the vertices that have appeared no later than the time $t$ and
% consisting of its source node $v_i$, its destination node $u_i$ and its occurrence time $t_i$. Here, the type of this edge can be represented by $(v_i, u_i)$ while the $t_i$ 
% that represents when the edge $(v_i, u_i)$ appears in $G_t$. Note that each ty


% Basical 


% Note that in this graph $G$, the node set may increase with respect to the time $t$ because 



% Consider a time-evolving graph $G_t = \{V_t, \mathcal{E}_t\}$. Let $V_t$ denote the node set of $G_t$ at time $t$, which includes all nodes that have been appeared no later than $t$.


% LetE={e1,e2,···}be  a  stream  of  edges  from  a  time-evolving  graphG.  Each  arriving  edge  is  a  tupleei= ui,vi,ti)consisting of a source nodeui∈ V, a destina-tion nodevi∈ V, and a time of occurrenceti, which is thetime at which the edge was added to the graph. For example,in a network traffic stream, an edgeeicould represent a con-nection made from a source IP addressuito a destinationIP addressviat timeti. We do not assume that the set ofverticesVis known a priori: for example, new IP addressesor user IDs may be created over the course of the stream


Regarding the code
\begin{itemize}
    \item What is ``alpha''?
    \item How to explain ``del-time'' well?
    \item Is ``directed-flag'' always true?
    \item what is ``negative-sampling-strategy''?
    \item Take care of ``node-level-flag'' and ``node-eval-interval''.
\end{itemize}
\begin{itemize}
    \item What is ``data-point.del-time-s, data-point.del-time-t''?
\end{itemize}
\begin{itemize}
    \item setup window $W$.
    \item If we set the forget parameter as $\delta$, the currently time-variance frequency becomes $\delta\sum_{t_i \leq T} w_{t_i}\exp(-\delta(T-t_i))$, decay: if freq < threshold, we remove this edge. Note that the $\delta$ should be relevant to $W$.
    \item Also record the last-time $T'$ to update an event...
    \item negative sample with negative weights: when to use online or setup?
    \item first update the previous model, then eval and then update memory 
    \item neighbor sample 
\end{itemize}

\begin{itemize}
\item $\mathbb{P}(f) = \frac{1}{\lambda}\exp(-\frac{f}{\lambda})$, $\lambda = \langle h_s, h_t \rangle_Q$ split two parts for frequent computation (support from the applied statistic paper~\cite{heard2010bayesian})
\item $\mathbb{P}(f) = \frac{1}{\sum_v\lambda}\exp(-\frac{f}{\sum_v\lambda})$
\item Difference from point process: more robust, average of time; different from poisson factorization -> over emphasize the large counts that check factors to cause imbalanced embedding 
\item Compared to statistical based -> factorization, community 
\item How to control online: 1) local update; 2) throw away property; 3) if no events, -> no anomaly...
\item Number of embedded nodes $1/(-\log f_{\min})^d$
\item How to detect community change? How to provide $p$ values? How to prove star anomaly?
\end{itemize}

